Building Open-Ended Embodied Agent via Language-Policy Bidirectional Adaptation

Building embodied agents on integrating Large Language Models (LLMs) and Reinforcement Learning (RL) have revolutionized human-AI interaction: researchers can now leverage language instructions to plan decision-making for open-ended tasks. However, existing research faces challenges in meeting the requirement of open-endedness. They typically either train LLM/RL models to adapt to a fixed counterpart, limiting exploration of novel skills and hindering the efficacy of human-AI interaction. To this end, we present OpenPAL, a co-training framework comprising two stages: (1) fine-tuning a pre-trained LLM to translate human instructions into goals for planning, and goal-conditioned training a policy for decision-making; (2) co-training to align the LLM and policy, achieving instruction open-endedness. We conducted experiments using Contra, an open-ended FPS game, demonstrating that an agent trained with OpenPAL not only comprehends arbitrary instructions but also exhibits efficient execution. These results suggest that OpenPAL holds the potential to construct open-ended embodied agents in practical scenarios.

==> sections/relatedwork.tex <==
\section{Related Work}
This work builds heavily upon the ideas of many related works. We now review some of these in the areas of goal-conditioned reinforcement learning, open-ended learning, human-AI interaction, and LLM-based ....

\paragraph{Goal-conditioned Reinforcement Learning}
Training goal-conditioned agents is a long-standing topic in reinforcement learning~\citep{plappert2018multi,liu2022goal}, originating from hierarchical reinforcement learning (HRL)~\citep{vezhnevets2017feudal,dayan1993improving,pateria2021hierarchical} to resolve the sparse rewarding challenge via decoupling end-to-end learning into multiple levels.
The most significant difference between these two close frameworks is whether the goal generator (or \emph{the Manager} in HRL) uses direct rewarding to improve goal generation.
In comparison, GRL uses implicit rewarding via UVFA~\citep{schaul2015universal}, a value function that takes input as a joint space of state and goal.
The goal representation in GRL is still an open question, generally determined by the task to be resolved.
We summarize the most popular categories as vector-based~\citep{florensa2018automatic,ren2019exploration,nair2018overcoming,fang2019curriculum,pitis2020maximum}, vision-based~\citep{campero2020learning,nair2019hierarchical,warde2018unsupervised,mendonca2021discovering,bousmalis2023robocat,groth2021goal} and text-based~\citep{brohan2023can,lynch2020language}.
In this work, we shape the goal space as a structured vector.
Sampling efficiency, or sparse rewarding in equivalent, is a critical challenge that GRL faces, and solutions to its research can be categorized into reward shaping~\citep{ng1999policy,ecoffet2021first,ding2023magnetic} and hindsight relabelling~\citep{andrychowicz2017hindsight,fang2019curriculum,zheng2022online}.
Reward shaping is a straightforward and efficient idea to address the sparse rewarding problem, while it relies on domain knowledge and complex feature engineering.
Hindsight relabelling is inspired by \cite{schaul2015prioritized}, which introduces a prioritized replay mechanism to improve the sample efficiency of RL methods.

\paragraph{Open-ended Learning}
There are too many categories for the research of open-ended learning, for instance, population-based learning~\citep{team2021open,jaderberg2019human}, empirical game theoretical analysis~\citep{balduzzi2019open,sukhbaatar2018intrinsic}, and curriculum reinforcement learning~\citep{narvekar2020curriculum}.
The most related to our work is the latter.
The research on curriculum reinforcement learning comprises several different paradigms~\citep{weng2020curriculum}, i.e., task-specific curriculum~\citep{akkaya2019solving,weinshall2018curriculum,bengio2009curriculum}, teacher-guided curriculum~\citep{portelas2020teacher,graves2017automated}, curriculum goal generation~\citep{racaniere2019automated,florensa2018automatic}, skill-based curriculum~\citep{jabri2019unsupervised}, and curriculum through distillation~\citep{rusu2017sim,czarnecki2018mix}.
In this work, we implemented open-ended learning as curriculum goal generation.
Along this line of research, there are two aspects that the community concentrates on, including (1) improving the coverage of goal space the policy performs and (2) scheduling the discovery of novel goals.
For instance, \cite{pmlr-v119-pong20a} and \cite{campos2020explore} propose to explore novel goals by maximizing state coverage.
\cite{nair2018visual} achieve that by leveraging VAE to learn a representation that generalizes the goal space.
To schedule the discovery of novel goals, \cite{florensa2018automatic} leverage LSGAN (Least-Squared GAN)~\citep{mao2017squares} that controls the generation of goals by learning a distribution correlates the set of goals at the appropriate level of difficulty.
With the promotion of training, LSGAN could gradually expand the distribution for goal generation.
\cite{zhang2020automatic} and \cite{zhao2020energybased} propose variants of Hindsight Replay Buffer~\citep{andrychowicz2017hindsight} to overcome the inefficiency of random goal exploration.
Specifically, \cite{zhang2020automatic} explicitly models the distribution of goal space via corresponding it to the standard deviation of multi-head Q values.
Then, the changing of the distribution implies the scheduling of goal exploration.
\cite{zhao2020energybased} propose an energy-based framework for prioritized exploration of novel goals.

\paragraph{Human-AI Interaction}
Our work is highly related to human-AI interaction (or human-AI coordination/collaboration).
This is a field that has been researched for a long time, and much work focuses on achieving collaboration by planning and learning with human behavior models~\citep{nikolaidis2013humanrobot,sadigh2016planning,swamy2020utility,carroll2020utility}, or seeking human equilibrium distinguished from multi-agent cases~\citep{10.1145/3306618.3314268,meta2022human}.
Some trials also leverage LLMs to translate human purpose into natural language instructions to achieve this target, e.g., \cite{pmlr-v202-hu23e} utilize LLMs to guide equilibrium learning.
The generalization capability could be a key to human-AI interaction, as we want an agent to collaborate with arbitrary humans. Thus, a lot of work concentrates on training a best-response policy to a diverse set of human-like policies so that the agent may generalize to unseen humans~\citep{cui2023adversarial,strouse2022collaborating,charakorn2022generating}.
In our work, an agent acquires the generalization capability by achieving open-endedness in the goal space.

\paragraph{Large Language Models for Agent Planning}
Recent efforts can be roughly classified into two groups. 1) Large language models for robot learning: Many prior works apply LLMs to generate subgoals for robot planning~\citep{brohan2023can,huang2022language}; (2) Large language models for text agents.
For (1), Inner Monologue~\citep{huang2023inner} incorporates environment feedback for robot planning with LLMs. Code as Policies~\citep{liang2022code} and ProgPrompt~\cite{singh2022progprompt} directly leverage LLMs to generate executable robot policies. VIMA~\citep{jiang2022vima} and PaLM-E~\citep{driess2023palm} fine-tune pre-trained LLMs to support multimodal prompts;
for (2), ReAct~\citep{yao2022react} leverages chain-of-thought prompting and generates both reasoning traces and task-specific actions with LLMs. Reflexion~\citep{shinn2023reflexion} is built upon ReAct with self-reflection to enhance reasoning.



==> sections/tables/cot_gpt4_prompt.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|p{13.5cm}|}
\hline
In order to complete the command `You should lie in wait', let us plan the states of the agent step by step using the following template:    \\ \hline
1. Analyze the verbal orders of teammates and players, what do you want to do? According to the command, also analysis the relevant states of teammates and enemies that need attention. \\
The verbal command of the teammate player is {[}Command{]}, which means teammate player wants the agent...        \\ \hline
2. Analyze which states of the agents are most relevant to the verbal commands of teammate player. The agents in the unselected states will adjust themselves to complete your plan (analyze the reason first, then select key states one by one as few as possible and as important as possible according to the degree of importance)?  \\
According to the teammate's command:  \\
2.1. {[}Reason1{]}: {[}State1{]}  \\
2.2. {[}Reason2{]}: {[}State2{]}  \\
...                     \\ \hline
3. Plan how these key states need to be adjusted (analyze the reason first, and then make adjustments one state by one state, the state can be changed or remain the same, and must be selected from the value range of the game state {[}Choice 1, Choice 2, ...{]})?  \\
According to the teammate's command:  \\
3.1. {[}State1{]}: {[}Reason1{]}: {[}Current\_value1{]} -\textgreater {[}Target\_value2{]}  \\
3.2. {[}State2{]}: {[}Reason2{]}: {[}Current\_value1{]} -\textgreater {[}Target\_value2{]}  \\
...          \\ \hline
4. Modify the adjustment that may be wrong, and refer to the Rules to analyze which state adjustments may conflict, repeat or be unnecessary, and output the modified adjustment plan:  According to the states adjustments in 3...  \\
4.1. {[}State1{]}: {[}Current\_value1{]} -\textgreater {[}Target\_value2{]}  \\
4.2. {[}State2{]}: {[}Current\_value1{]} -\textgreater {[}Target\_value2{]}  \\
...                      \\ \hline
5. According to the analyze and the planing of the verbal command, further analyze the behavior tendency required in the adjustment process (the proportion of Mobile, Offense, Waiting, Supplies, Scouting, first analyze the reason, and then calculate the percentage)  \\
Mobile: {[}Reason1{]}: {[}Percent1{]}  \\
Offense: {[}Reason2{]}: {[}Percent2{]}  \\
Waiting: {[}Reason3{]}: {[}Percent3{]}  \\
Supplies: {[}Reason4{]}: {[}Percent4{]}  \\
Scouting: {[}Reason5{]}: {[}Percent5{]}           \\ \hline
6. Analyze how long the current command needs to be kept (for example, the command of `killing the enemy' needs to be kept for a `short term', and the command of `pay attention to reconnaissance' needs to be kept for a `long term'. First analyze the reason and then make a judgment).  \\
According to the command of the teammate, {[}Analysis{]}: The current command needs to be kept by `{[}XX term{]}'.   \\
If you see phrases like {[}Context{]} in answer template, replace the entire phrase according to the meaning of the Context, do not repeat the content; make analogy expansion for `...'; keep `:'; absolutely do not modify others in template. \\ \hline
\end{tabular}
% }
\caption{Chain of thought prompt for GPT4.}
\label{tab_gpt4_prompt}
\end{table}

==> sections/tables/cot_gpt4_response.tex <==
\begin{table}[h]
\centering

\begin{tabular}{|p{13.5cm}|}
\hline

    1. Analyze the verbal orders of teammates and players, what do you want to do? According to the command, also analysis the relevant states of teammates and enemies that need attention.\\
     The verbal command of the teammate player is `You should lie in wait', which means teammate player wants the agent to set up an ambush or take a hiding position. \\    \hline
2. Analyze which states of the agents are most relevant to the verbal commands of teammate player. The agents in the unselected states will adjust themselves to complete your plan.\\
     According to the teammate`S command:\\
     2.1. Need to hide: `Whether prone position', `Whether crouch position'\\
     2.2. Reduce movement to stay unnoticed: `Average velocity', `Length of distance moved'\\
     2.3. Ensure readiness for potential attack: `Whether hold a gun'    \\ \hline
3. Plan how these key states need to be adjusted.\\
     According to the teammate`S command:\\
     3.1. `Whether prone position': Need to hide: `False' -\textgreater{}   `True'\\
     3.2. `Whether crouch position': Alternative hiding posture if not prone: `False' -\textgreater{}   `True'\\
     3.3. `Average velocity': Reduce movement: `Fast' -\textgreater{}   `Static'\\
     3.4. `Length of distance moved': Reduce movement: `Short' -\textgreater{}   `No movement'\\
     3.5. `Whether hold a gun': Ensure readiness for potential attack: `True' -\textgreater{}   `True'\\      \hline
4. Modify the adjustment that may be wrong, and refer to the Rules to analyze which state adjustments may conflict, repeat or be unnecessary, and output the modified adjustment plan:\\
     According to the states adjustments in 3:\\
     4.1. `Whether prone position': `False' -\textgreater{} `True'\\
     4.2. `Average velocity': `Fast' -\textgreater{} `Static'\\
     4.3. `Length of distance moved': `Short' -\textgreater{} `No movement'\\
     4.4. `Whether hold a gun': `True' -\textgreater{} `True'\\
     (Removed `Whether crouch position' as it conflicts with `Whether prone position' and prone position gives better cover for an ambush.)\\    \hline
5. According to the analyze and the planing of the verbal command, further analyze the behavior tendency required in the adjustment process.\\
     Mobile: Need to stop all movement: 0\%\\
     Offense: Must be ready to attack if necessary: 20\%\\
     Waiting: The main goal is to set up an ambush and wait: 70\%\\
     Supplies: No need for supplies during this phase: 0\%\\
     Scouting: Need to observe the surroundings, but not actively scout: 10\%\\   \hline
6. Analyze how long the current command needs to be kept.\\
     According to the command of the teammate, taking a hiding position or setting up an ambush is usually done with the intention of waiting for an opportune moment to strike or observe the enemy`S movement: The current command needs to be kept by `long term'.  \\ \hline


\end{tabular}

\caption{Chain of thought response from GPT4.}
\label{tab_gpt4_response}
\end{table}

==> sections/tables/prompt_and_response.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|}
\hline
\multirow{6}{*}{prompt} & \begin{tabular}[c]{@{}l@{}}system\\ background\\ prompt\end{tabular} & \begin{tabular}[c]{@{}l@{}}We have an agent and a player working together as a teammate in a \\ PUBG game. We hope you can help the agent plan how the agent's\\ game state should change, so as to complete the player's command and\\ help the player win the game.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \cline{2-3} 
                        & \begin{tabular}[c]{@{}l@{}}teammate\\ state\\ prompt\end{tabular}    & \begin{tabular}[c]{@{}l@{}}The state of the agent's teammates can be described as follows:\{`\\ Length of distance moved': `No movement', `Average velocity': `Slow',\\ `Horizontal direction of movement': `Southeast', `Horizontal \\ direction of view': `South', `Pitch direction of view': `Medium', \\ `Health level': `Empty', `Whether to restore health': `False', \\ `Whether the health is damaged': `False', `Whether rescued teammate':\\  `False', `Whether prone position': `False', `Whether crouch \\ position': `False', `Whether have a gun': `True', `Whether hold a \\ gun': `False', `Whether have bullets': `True', `Whether have medical\\ kits': `True', `Whether be knocked down': `False', `Damage to enemy': \\ `Zero', `Whether knock down enemy': `False', `Whether seen enemy': \\ `True', `Number of enemies have ever seen': 5, `Whether seen by \\ enemy': `True', `Distance with nearest enemy': `Nearby', `Whether \\ closer with nearest enemy': `False', `ID of teammate player': 2\}\end{tabular}                                                                                                                                                                                                                                                                                                                                                              \\ \cline{2-3} 
                        & \begin{tabular}[c]{@{}l@{}}enemy\\ state\\ prompt\end{tabular}       & \begin{tabular}[c]{@{}l@{}}The state of the enemy can be described as follows:\{`Horizontal \\ direction of movement of enemy': `Southwest', `Velocity of enemy':\\ `Slow', `Enemy's position relative to agent': `West'\}\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \cline{2-3} 
                        & \begin{tabular}[c]{@{}l@{}}self\\ state\\ prompt\end{tabular}        & \begin{tabular}[c]{@{}l@{}}The state of the agent can be described as follows:\{`Damage to \\ enemy': `Zero', `Whether knock down enemy': `False', `Whether kill \\ enemy': `False', `Whether seen enemy': `True', `Whether seen by \\ enemy': `True', `Number of enemies have ever seen': 3, `Length of \\ distance moved': `Short', `Average velocity': `Fast', `Horizontal \\ direction of movement': `West', `Horizontal direction of view': \\ `NorthEast', `Pitch direction of view': `Medium', `Health level': \\ `Full', `Whether to restore health': `False', `Whether the health is\\  damaged': `False', `Whether rescued teammate': `False', `Whether be\\  knocked down': `False', `Whether prone position': `False', `Whether\\  have a gun': `True', `Whether have bullets': `True', `Whether have \\ medical kits': `True', `Distance with nearest enemy': `Nearby', \\ `Whether closer with nearest enemy': `True', `Whether crouch \\ position': `False', `Whether hold a gun': `True', `Whether seen by \\ teammate': `True', `Length of distance from agent to teammate': \\ `Touch', `Teammate's position relative to agent': `Southwest', \\ `Whether follow with the views of teammate': `False', `Whether \\ target the same enemy as teammate': `False', `Whether follow with \\ the movement direction of teammate': `False'\}\end{tabular} \\ \cline{2-3} 
                        & \begin{tabular}[c]{@{}l@{}}command\\ prompt\end{tabular}             & \begin{tabular}[c]{@{}l@{}}Teammate player gives you a verbal command based on the current\\ game states:`You should lie in wait.'\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \cline{2-3} 
                        & \begin{tabular}[c]{@{}l@{}}question\\ prompt\end{tabular}            & \begin{tabular}[c]{@{}l@{}}In order to complete the command `You should lie in wait.', how\\ the agent's game state should change?\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \hline
response                & \begin{tabular}[c]{@{}l@{}}goal\\ meta-state\\ prompt\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Whether prone position:True\\ Average velocity:Static\\ Length of distance moved:No movement\\ Whether hold a gun:True\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\end{tabular}
\caption{\textbf{Example of prompt and response.}}
\label{tab_prompt}
\end{table}
